Correlation in Neuronal Calcium Spiking: Quantification based on Empirical Mutual Information Rate

Quantification of neuronal correlations in neuron populations helps us to understand neural coding rules. Such quantification could also reveal how neurons encode information in normal and disease conditions like Alzheimer's and Parkinson's. While neurons communicate with each other by transmitting spikes, there would be a change in calcium concentration within the neurons inherently. Accordingly, there would be correlations in calcium spike trains and they could have heterogeneous memory structures. In this context, estimation of mutual information rate in calcium spike trains assumes primary significance. However, such estimation is difficult with available methods which would consider longer blocks for convergence without noticing that neuronal information changes in short time windows. Against this backdrop, we propose a faster method that exploits the memory structures in pair of calcium spike trains to quantify mutual information shared between them. Our method has shown superior performance with example Markov processes as well as experimental spike trains. Such mutual information rate analysis could be used to identify signatures of neuronal behavior in large populations in normal and abnormal conditions.

==> section/Spike_Train_Inference.tex <==
\section{Spike train inference}
\label{sec:append}
To infer spike train from time course of normalized fluorescence intensity, we used a fast nonnegative deconvolution algorithm assuming a linear relation between fluorescence intensity and calcium concentration subject to baseline offset and normal error. Specifically, we modeled the fluorescence measurement $F_t$ of any neuron (whose index $i$ is dropped for the sake of convenience) at time $t$ to be proportional to intracellular calcium concentration $C_t$:
%\begin{small}
\begin{equation}
F_t =\alpha C_{t} +\beta +\varepsilon_t,
\label{eq:1}
\end{equation} 
%\end{small} 
%\noindent 
where $\alpha$ denotes a sclae factor,  $\beta$  the baseline offset in calcium concentration of the cell, and the error $\varepsilon_{t} \sim iid ~N(0,\sigma^{2})$ at  time $t$ is zero mean Gaussian with standard deviation $\sigma$ and independently and identically distributed. Further,
the relation between calcium concentration at time $t$ and time $t-1$ is given by
%\begin{small}
\begin{equation}
C_t= (1-{\Delta}\mathbin{/}{\tau}) C_{t-1} + ({\Delta}\mathbin{/}{\tau}) C_{b}+ A n_t,
\label{eq:2}
\end{equation}
%\end{small}
where $\Delta$ is frame duration or 1/(frame rate) and associated number of spikes $n_t \sim iid \,\, Poisson ({\lambda} {\Delta})$ follows Poisson distribution with rate $\lambda$. The intracellular concentration raises by A $\mu$M for each spike and subsequently decays down to baseline concentration $C_b$ $\mu$M with time constant $\tau$.

Given the statistical model, the aim is to maximize posteriori probability of number of spikes $n_t$, given the fluorescence observations {\boldmath${F_t}$}:
%\begin{small}
\begin{equation}  
\hat{n} = \arg\max_{n_t \leq N_0 }  \ {{  \mbox {Pr} [n_t \vert F_t]}},
\label{eq:3}
\end{equation}
%\end{small}
where $N_0$ represents maximum possible number of spikes in a frame.
The inferred spiking rate vector $\hat{n}$ is thresholded for identifying the spikes. 

\textbf{Threshold selection}

In fast nonnegative deconvolution algorithm, the estimated spike rate indicate number of spikes at each time point. Unfortunately, such estimated spiking rates are generally noisy, and may lead to inference of erroneous spikes. We mitigated such errors in spike inference by setting an adaptive threshold on estimated spiking rate. Specifically, we chose the spiking threshold 
\begin{equation}  
P_{th} = 3 \sigma_p, 
\label{eq:threshold}
%\end{align}
\end{equation}
where $\sigma_p$ indicates standard deviation of inferred spiking rate vector $\hat{n}$. The instants where spiking rate is greater than spiking threshold, $P_{th}$ are set as binary one (high spiking) otherwise zero (low spiking). Such binary spike sequences used for further analysis.





==> section/ref.tex <==
\begin{thebibliography}{99}

\bibitem{c1} Y. Penn, M. Segal, and E. Moses, Network synchronization in hippocampal neurons, Proceedings of the National Academy of Sciences, Mar. 2016, 113(12), pp.3341-6.

\bibitem{c2} S. Zeng, B. Li, S. Zeng, S. Chen, Simulation of spontaneous Ca 2+ oscillations in astrocytes mediated by voltage-gated calcium channels, Biophysical journal, Nov. 2009, 97(9), pp.2429-37.
\bibitem{c3} M. Goldberg, M. De Pitta, V. Volman, H. Berry, E. Ben-Jacob, Nonlinear gap junctions enable long-distance propagation of pulsating calcium waves in astrocyte networks, PLoS Comput Biol,  Aug. 2010, 6(8), e1000909.
\bibitem{c4} D. J. O'Shea, E. Trautmann, C. Chandrasekaran, S. Stavisky , J. C. Kao, M. Sahani, S. Ryu, K. Deisseroth, K.V. Shenoy, The need for calcium imaging in nonhuman primates: New motor neuroscience and brain-machine interfaces, Exp Neurol, 2017, 287(Pt 4), pp. 437-451.
\bibitem{c5} J. Cichon, and W.B. Gan, Branch-specific dendritic Ca(2+) spikes cause persistent synaptic plasticity, Nature, 2015, 520(7546), pp.180-5.
\bibitem{c6} C. Y. Yang, A. J. Woolley, D. Tsai, G. J. Suaning, J. W. Morley, N. H. Lovell, Calcium Imaging of Retinal Ganglion Cell Dendritic Responses to Extracellular Microelectrode Stimulation, in 7th International IEEE/EMBS Conference on Neural Engineering (NER), Apr 2015, pp.438-441.
\bibitem{c7} M. Lavrentovich, S. Hemkin, A mathematical model of spontaneous calcium oscillations in astrocytes, J. Theoritical Biology, 2008, 251(4), pp.553-560.
\bibitem{c8}  S. Mennerick, and C. F. Zorumski, Presynaptic influence on the time course of fast excitatory synaptic currents in cultured hippocampal cells,The Journal of neuroscience,  Apr 1995, 15(4), pp.3178-92.
\bibitem{c9} L. Giri, A. K. Patel, W. A. Karunarathne, V. Kalyanaraman, K. V. Venkatesh, N. Gautam, A G-protein subunit translocation embedded network motif underlies GPCR regulation of calcium oscillations, Biophys J, 2014. 107(1), pp.242-54.
\bibitem{c10} J. T. Vogelstein,  A. M. Packer, T. A. Machado, T. Sippy, B. Babadi, R. Yuste, L. Paninski, Fast nonnegative deconvolution for spike train inference from population calcium imaging, Journal of neurophysiology, 2010, 104(6), pp.3691-3704.

\end{thebibliography}
